EFM3D: A Benchmark for Measuring Progress Towards 3D Egocentric Foundation Models

The advent of wearable computers enables a new source of context for AI that is embedded in egocentric sensor data. This new egocentric data comes equipped with fine-grained 3D location information and thus presents the opportunity for a novel class of spatial foundation models that are rooted in 3D space. To measure progress on what we term Egocentric Foundation Models (EFMs) we establish EFM3D, a benchmark with two core 3D egocentric perception tasks. EFM3D is the first benchmark for 3D object detection and surface regression on high quality annotated egocentric data of Project Aria. We propose Egocentric Voxel Lifting (EVL), a baseline for 3D EFMs. EVL leverages all available egocentric modalities and inherits foundational capabilities from 2D foundation models. This model, trained on a large simulated dataset, outperforms existing methods on the EFM3D benchmark.

==> tables/obb_ablation_old.tex <==
%\begin{table}[]
%    \centering
%    \begin{tabular}{c|c|c| c|c|c|c|}
%         rgb & slams & points    & ASE mAP & ASE mAP & AO3D mAP \\ 
%        & &                      & Snippet  & Sequence  &   Sequence  \\ \hline           
%          & & \cmark             & 0.27 & 0.59 & 0.45 \\
%        \cmark & &               & 0.30 & 0.66 & \TODO{0.36} \\
%          & \cmark &             & 0.33 & 0.71 & 0.41 \\
%        \cmark  & \cmark &       & 0.36 & 0.72 & \TODO{0.37} \\
%        \cmark & & \cmark        & 0.42 & 0.78 & \TODO{0.40} 0.44? \\
%          & \cmark & \cmark      & 0.43 & 0.79 & 0.45 \\
%        \cmark & \cmark & \cmark & 0.45 & 0.80 & \TODO{0.41} \\
%    \end{tabular}
%    \caption{We ablate different input modalities for \EFMmodel{}: rgb video snippets, left and right slam stream snippets and semidense points. }
%    \label{tab:obj_ablation}
%\end{table}

\begin{table}[]
    \centering
    % https://docs.google.com/spreadsheets/d/1-C4hIRjXC9phLz-k_BGhe0bWYeCYPMVtjMZgcpshQFs/edit#gid=789119799

    % after joint mAP computation for all but snippet results
    % TODO update the snippet results 
    \begin{tabular}{c|c|c| c|c|c|c|c| c|c|c|}
         rgb   & greys  & points & free  & agg.  & agg.  & aug   & aug   & \ASE{} mAP & \ASE{} mAP & \AOThree{} mAP \\ 
               &        &        &       & mean  & std   & geom  & photo & Snippet  & Sequence  &   Sequence  \\ \hline           
               &        & \cmark &       &\cmark &       &       &       & 0.24 & 0.42 & 0.19 \\
        \cmark &        &        &       &\cmark &       &       &       & 0.26 & 0.52 & 0.13 \\
               & \cmark &        &       &\cmark &       &       &       & 0.29 & 0.58 & 0.13 \\
        \cmark & \cmark &        &       &\cmark &       &       &       & 0.31 & 0.62 & 0.15 \\  
    %   \cmark & \cmark &        &       &\cmark &       &       &       & 0.32 & 0.61 & 0. \\  % with compression of features
        \cmark &        & \cmark &       &\cmark &       &       &       & 0.38 & 0.72 & 0.22 \\
               & \cmark & \cmark &       &\cmark &       &       &       & 0.39 & 0.73 & 0.25 \\
        \cmark & \cmark & \cmark &       &\cmark &       &       &       & 0.40 & 0.75 & 0.22 \\ \hline
        \cmark &        & \cmark &       &       &\cmark &       &       & 0.37 & 0.66 & 0.21 \\
        \cmark &        & \cmark &       &\cmark &\cmark &       &       & 0.39 & 0.71 & 0.23 \\ \hline
        \cmark &        & \cmark &       &\cmark &       &\cmark &       & 0.38 & 0.67 & 0.25 \\
        \cmark &        & \cmark &       &\cmark &       &\cmark &\cmark & 0.38 & 0.68 & 0.23 \\ \hline
        \cmark &        &        &\cmark &\cmark &       &       &       &\todo & 0.69 & 0.23 \\
        \cmark &        & \cmark &\cmark &\cmark &       &       &       &\todo & 0.71 & 0.26 ›\\

    %   \cmark & \cmark & \cmark & 0.41 & 0.75 & 0.  \\ # with compression
    \end{tabular}
    \caption{We ablate different input modalities for \EFMmodel{}: RGB video, left and right grey-scale streams and semidense points. }
    \label{tab:obj_modality_ablation}
\end{table}


\begin{table}[]
    \centering
    % https://docs.google.com/spreadsheets/d/1-C4hIRjXC9phLz-k_BGhe0bWYeCYPMVtjMZgcpshQFs/edit#gid=789119799
    \begin{tabular}{c|c|c|c|c|}
        geom. aug. & photo aug. & \ASE{} mAP & \ASE{} mAP & \AOThree{} mAP \\ 
                   &            & Snippet  & Sequence  &   Sequence  \\ \hline           
                   &            & 0.26 & 0.52 & 0.13 \\
        \cmark     &            & 0.38 & 0.67 & 0.25 \\
        \cmark     &    \cmark  & 0.38 & 0.68 & 0.23 \\
    \end{tabular}
    \caption{We ablate training with augmentations for \EFMmodel{}. With RGB stream and points input.}
    \label{tab:obj_aug_ablation}
\end{table}


\begin{table}[]
    \centering
    % https://docs.google.com/spreadsheets/d/1-C4hIRjXC9phLz-k_BGhe0bWYeCYPMVtjMZgcpshQFs/edit#gid=789119799
    \begin{tabular}{c|c|c|c|c|c|}
         pts   & free    & \ASE{} mAP & \ASE{} mAP & \AOThree{} mAP \\ 
               &           & Snippet  & Sequence  &   Sequence  \\ \hline   
        %       &           & 0.26 & 0.52 & 0.13 \\
        \cmark &           & 0.38 & 0.72 & 0.22 \\
               & \cmark    &\todo & 0.69 & 0.23 \\
        \cmark & \cmark    &\todo & 0.71 & 0.26 \\
        % compress mean \& std    & 0.39 & 0.72 & 0.33 \\
    \end{tabular}
    \caption{We ablate the use of points and freespace masks for the \EFMmodel{}. With RGB stream as the base input. }
    \label{tab:obj_freespace_ablation}
\end{table}



%\begin{table}[]
%    \centering
%    \begin{tabular}{c|c|c| c|c|c|c|}
%         rgb & slams & points    & \ASE{} mAP & \ASE{} mAP & \AOThree{} mAP \\ 
%        & &                      & Snippet  & Sequence  &   Sequence  \\ \hline           
%        \cmark & &               & 0.30 & 0.66 & \TODO{0.36} \\
%        \cmark  & \cmark &       & 0.36 & 0.72 & \TODO{0.37} \\
%        \cmark & & \cmark        & 0.42 & 0.78 & \TODO{0.40} 0.44? \\
%          & \cmark &             & 0.33 & 0.71 & 0.41 \\
%        \cmark & \cmark & \cmark & 0.45 & 0.80 & \TODO{0.41} \\
%          & & \cmark             & 0.27 & 0.59 & 0.45 \\
%          & \cmark & \cmark      & 0.43 & 0.79 & 0.45 \\
%    \end{tabular}
%    \caption{We ablate different input modalities for \EFMmodel{}: rgb video snippets, left and right slam stream snippets and semidense points. }
%    \label{tab:obj_ablation}
%\end{table}

==> tables/surf_datasets.tex <==

\begin{table}[]
    \centering
    \begin{tabular}{c|c|c}
           & \# scenes & \# OBBs  \\ \hline
        \ASE{} &  & \\
        \ADT{} &  & \\
        Omni3d & & \\
        ScanNet & & \\
        Replica & & \\
    \end{tabular}
    \caption{The ASE dataset is a large scale dataset for 3D perception.\TODO{maybe collapse with Table1}}
    \label{tab:surf_datasets}
\end{table}

==> tables/surf_eval_old.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{c|c|c}
           & ASE & ADT  \\ \hline
        NeuralRecon & & \\
        SimpleRecon & &\\
        ZoeDepth & &\\
        OpenOcc & &\\
    \end{tabular}
    \caption{We show in domain performance on ASE validation dataset as well as sim-to-real generalization performance on the ADT dataset.}
    \label{tab:surf_perf}
\end{table}

\begin{table}[]
    \centering
    \begin{tabular}{c|c|c}
           & ASE & ADT  \\ \hline
        VegoNet only Points & &\\
        VegoNet only Features & &\\
        VegoNet & &\\
    \end{tabular}
        \begin{tabular}{c|c|c}
           & ASE & ADT  \\ \hline
        OpenOcc only Points & &\\
        OpenOcc only Features & &\\
        OpenOcc & &\\
    \end{tabular}
    \caption{We show that adding points and using frozen 2d foundation features helps.}
    \label{tab:surf_perf}
\end{table}


\begin{table}[]
\centering
\small
\begin{tabular}{|p{2cm}|l|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1.1cm}|}
\hline
Method     & Fusion        & Res (cm) & Acc. (cm) & Comp. (cm) & Prec @5cm & Recall @5cm & F-score @5cm\\ \hline
GT depth   & TSDF       & 4                     &                &                  &         &      &   \\ \hline
GT depth   & TSDF        & 1                     &                &                   &         &       &   \\ \hline
ZoeDepth   & TSDF       & 4                     &                &                  &         &      &   \\ \hline
ZoeDepth   & TSDF        & 1                     &                &                   &         &       &   \\ \hline
TCD        & TSDF & 4                      &                     &                        &               &            &         \\ \hline
TCD        & TSDF & 1                      &                     &                        &               &            &         \\ \hline
SimpleRecon & TSDF          & 4                      &                     &                        &               &            &         \\ \hline
SimpleRecon & TSDF          & 1                      &                     &                        &               &            &         \\ \hline
NeuralRecon & Volume          & 4                      &                     &                        &               &            &         \\ \hline

\end{tabular}
\caption{We show the 3D surface reconstruction performance of the state-of-the-art methods on on the ADT test dataset. All the methods are evaluated using the best off-the-shelf models.}
\end{table}

\begin{table}[]
\centering
\small
\begin{tabular}{|p{2cm}|l|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1.1cm}|}
\hline
Method     & Fusion        & Res (cm) & Acc. (cm) & Comp. (cm) & Prec @5cm & Recall @5cm & F-score @5cm\\ \hline
GT depth   & TSDF       & 4                     &                &                  &         &      &   \\ \hline
GT depth   & TSDF        & 1                     &                &                   &         &       &   \\ \hline
OpenOcc & Volume        & 6.25                     &                 &                    &          &      &    \\ \hline
OpenOcc \newline only Point & Volume        & 6.25                    &                 &                    &          &       &    \\ \hline
OpenOcc \newline only Features & Volume        & 6.25                    &                 &                    &          &       &    \\ \hline
NeuralRecon & Volume          & 4                     &                 &                   &          &       &    \\ \hline
SimpleRecon & TSDF          & 4                     &                 &                   &          &       &    \\ \hline
SimpleRecon & TSDF          & 1                     &                 &                   &          &       &    \\ \hline


\end{tabular}
\caption{We show the in-domain 3D surface reconstruction performance on the ASE dataset. All the methods are trained and evaluated on the simulated ASE dataset.}
\end{table}

\begin{table}[]
\centering
\small
\begin{tabular}{|p{2cm}|l|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1.1cm}|}
\hline
Method     & Fusion        & Res (cm) & Acc. (cm) & Comp. (cm) & Prec @5cm & Recall @5cm & F-score @5cm\\ \hline
GT depth   & TSDF       & 4                     &                 &                   &          &       &    \\ \hline
GT depth   & TSDF        & 1                     &                 &                    &          &       &    \\ \hline
OpenOcc & Volume        & 6.25                     &                 &                    &          &      &    \\ \hline
OpenOcc \newline only Point & Volume        & 6.25                    &                 &                    &          &       &    \\ \hline
OpenOcc \newline only Features & Volume        & 6.25                    &                 &                    &          &       &    \\ \hline
NeuralRecon & Volume          & 4                     &                 &                   &          &       &    \\ \hline
SimpleRecon & TSDF          & 4                     &                 &                   &          &       &    \\ \hline
SimpleRecon & TSDF          & 1                     &                 &                   &          &       &    \\ \hline

\end{tabular}
\caption{We show the sim-to-real 3D surface reconstruction performance on the ASE dataset. All the methods are trained on the simulated ASE dataset and evaluated on the real ADT dataset.}
\end{table}

\begin{table}[]
\centering
\small
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
Method             & VoxRes (cm) & Acc. (cm) & Comp. (cm) & Prec@5cm & Recall@5cm & F-score \\ \hline
GT depth           & 4                     & 2.03                & 11.83                  & 0.902         & 0.554      & 0.686   \\ \hline
GT depth           & 1                     & 1.47                & 6.31                   & 0.957         & 0.691      & 0.802   \\ \hline
Zoe depth          & 4                     & 50.06               & 61.05                  & 0.227         & 0.119      & 0.153   \\ \hline
Zoe depth          & 1                     & 41.77               & 74.12                  & 0.235         & 0.075      & 0.109   \\ \hline
TCD &                       &                     &                        &               &            &         \\ \hline
TCD &                       &                     &                        &               &            &         \\ \hline
SimpleRecon           & 4                     & ?                & ?                  & ?         & ?      & ?   \\ \hline
SimpleRecon           & 1                     & ?                & ?                  & ?         & ?      & ?   \\ \hline

\end{tabular}
\caption{\TODO{\textbf{BACKUP}}:We show the 3D surface reconstruction performance for depth fusion based methods on ADT validation dataset.}
\end{table}
